The Lick-Carnegie Exoplanet Survey: HD32963 -- A New Jupiter Analog Orbiting a Sun-like Star

We present a set of 109 new, high-precision Keck/HIRES radial velocity (RV) observations for the solar-type star HD 32963. Our dataset reveals a candidate planetary signal with a period of 6.49 $\pm$ 0.07 years and a corresponding minimum mass of 0.7 $\pm$ 0.03 Jupiter masses. Given Jupiter's crucial role in shaping the evolution of the early Solar System, we emphasize the importance of long-term radial velocity surveys. Finally, using our complete set of Keck radial velocities and correcting for the relative detectability of synthetic planetary candidates orbiting each of the 1,122 stars in our sample, we estimate the frequency of Jupiter analogs across our survey at approximately 3%.

==> refs.tex <==
\bibitem[Moutou et  
 al.(2011)]{Moutou2011} Moutou, C., Mayor, M., Lo Curto, G., et al.\ 2011, \aap, 527, A63  
  
  

\bibitem[Wright et al.(2011)]{Wright2011} Wright, J.~T., Veras,  
 D., Ford, E.~B., et al.\ 2011, \apj, 730, 93  
  
  

\bibitem[Bonfils et  
 al.(2013)]{Bonfils2013} Bonfils, X., Delfosse, X., Udry, S., et al.\ 2013, \aap, 549, A109  
  
  

\bibitem[Wright et al.(2009)]{Wright2009} Wright, J.~T., Upadhyay,  
 S., Marcy, G.~W., et al.\ 2009, \apj, 693, 1084  
  
  

\bibitem[Butler et al.(2006)]{Butler2006} Butler, R.~P., Wright,  
 J.~T., Marcy, G.~W., et al.\ 2006, \apj, 646, 505  
  
  

\bibitem[Fischer et al.(2009)]{Fischer2009} Fischer, D., Driscoll,  
 P., Isaacson, H., et al.\ 2009, \apj, 703, 1545  
  
  

\bibitem[Gregory  
 \& Fischer(2010)]{Gregory2010} Gregory, P.~C., \& Fischer, D.~A.\ 2010, \mnras, 403, 731  
  
  

\bibitem[Naef et  
 al.(2010)]{Naef2010} Naef, D., Mayor, M., Lo Curto, G., et al.\ 2010, \aap, 523, A15  
  
  

\bibitem[Naef et  
 al.(2010)]{Naef2010} Naef, D., Mayor, M., Lo Curto, G., et al.\ 2010, \aap, 523, A15  
  
  

\bibitem[Butler et al.(2006)]{Butler2006} Butler, R.~P., Wright,  
 J.~T., Marcy, G.~W., et al.\ 2006, \apj, 646, 505  
  
  

\bibitem[Wright et al.(2008)]{Wright2008} Wright, J.~T., Marcy,  
 G.~W., Butler, R.~P., et al.\ 2008, \apjl, 683, L63  
  
  

\bibitem[Bailey et al.(2009)]{Bailey2009} Bailey, J., Butler,  
 R.~P., Tinney, C.~G., et al.\ 2009, \apj, 690, 743  
  
  

\bibitem[Wittenmyer et al.(2014)]{Wittenmyer2014} Wittenmyer, R.~A.,  
 Horner, J., Tinney, C.~G., et al.\ 2014, \apj, 783, 103  
  
  

\bibitem[Boisse et  
 al.(2012)]{Boisse2012} Boisse, I., Pepe, F., Perrier, C., et al.\ 2012, \aap, 545, A55  
  
  

\bibitem[Pepe et  
 al.(2007)]{Pepe2007} Pepe, F., Correia, A.~C.~M., Mayor, M., et al.\ 2007, \aap, 462, 769  
  
  

\bibitem[Howard et al.(2010)]{Howard2010} Howard, A.~W., Johnson,  
 J.~A., Marcy, G.~W., et al.\ 2010, \apj, 721, 1467  
  
  

\bibitem[Jones et al.(2010)]{Jones2010} Jones, H.~R.~A., Butler,  
 R.~P., Tinney, C.~G., et al.\ 2010, \mnras, 403, 1703  
  
  


